Subspace Learning with Partial Information

The goal of subspace learning is to find a $k$-dimensional subspace of $\mathbb{R}^d$, such that the expected squared distance between instance vectors and the subspace is as small as possible. In this paper we study subspace learning in a partial information setting, in which the learner can only observe $r \le d$ attributes from each instance vector. We propose several efficient algorithms for this task, and analyze their sample complexity

==> header.tex <==
%\usepackage{graphicx,subfigure}
%\usepackage{epsfig}
\usepackage{hyperref}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{algorithm}
\usepackage{algorithmic}
%\usepackage{url}
%\usepackage{enumerate}
%\usepackage{amsfonts}
%\usepackage{boxedminipage}
%\usepackage{xcolor}
% \usepackage{framed}  
%\usepackage{rotating}
%\usepackage{array}
%\usepackage{multirow}
%\usepackage{color}
\usepackage{tikz}
\usepackage{subfig}
%\usepackage{mathabx}
%\usepackage{ragged2e,booktabs,caption}
%\usepackage{amsthm}
%\usepackage{empheq}




% theorems with small letters
%\newtheorem{definition}{Definition}
%\newtheorem{lemma}{Lemma}
%\newtheorem{corollary}{Corollary}
%\newtheorem{theorem}{Theorem}
% \newtheorem{proposition}{Proposition}
% \newtheorem{assumption}{Assumption}
%\newtheorem{example}{Example}
%\newtheorem*{proof*}{Proof}
% \newtheorem{exercise}{Exercise}
%\newtheorem{remark}{Remark}
%\newtheorem{claim}{Claim}

% bf - letters
\newcommand{\bx}{{\mathbf x}}
\newcommand{\by}{{\mathbf y}}
\newcommand{\bz}{{\mathbf z}}
\newcommand{\bw}{{\mathbf w}}
\newcommand{\bv}{{\mathbf v}}
\newcommand{\bu}{{\mathbf u}}
\newcommand{\be}{{\mathbf e}}
\newcommand{\br}{{\mathbf{r}}}
\newcommand{\bsig}{{\mathbf \sigma}}

%bf - numbers
\newcommand{\bzero}{{\mathbf{0}}}

% bf - expressions
\newcommand{\rV}{{\mathbf {Var}}}


% mathbb
\newcommand{\prob}{Pr}
\newcommand{\bE}{\,\mathbb{E}}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\realspos}{\mathbb{R}_{\geq 0}}
\newcommand{\realsneg}{\mathbb{R}_{\leq 0}}
\newcommand{\bN}{\mathbb{N}}
\newcommand{\bZ}{\mathbb{Z}}
\newcommand{\bC}{\mathbb{C}}
\newcommand{\bQ}{\mathbb{Q}}
\newcommand{\bB}{\mathbb{B}}

% bars
\newcommand{\barw}{\bar{\w}}
\newcommand{\barF}{\bar{F}}
\newcommand{\barlambda}{\bar{\lambda}}
\newcommand{\barA}{\bar{A}}
\newcommand{\barI}{\bar{I}}

%mathrm
\newcommand{\sgn}{{\mathrm{sgn}}}
\newcommand{\rank}{\mathrm{rank}}
\newcommand{\supp}{\mathrm{supp}}
\newcommand{\spn}{\mathrm{span}}
\newcommand{\image}{\mathrm{image}}
\newcommand{\tr}{{\mathrm{tr}}}
\newcommand{\diag}{{\mathrm{diag}}}
\newcommand{\T}{\mathrm{time}}
\newcommand{\sig}{\mathrm{sig}}
\newcommand{\poly}{\mathrm{poly}}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\thalf}{\tfrac{1}{2}}
\newcommand{\eqdef}{\stackrel{\mathrm{def}}{=}}
\newcommand{\opt}{\mathrm{opt}}
\newcommand{\Var}{\mathrm{Var}}


%  mathcal
\newcommand{\cF}{{\mathcal F}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cE}{\mathcal{E}}

% miscellaneous
\newcommand{\mathcomment}[1]{\color{red}{\textbf{#1}}}
%\newenvironment{proof}{\par\noindent{\bf Proof\ }}{\hfill\BlackBox\\[2mm]}
%\newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}}  
\newcommand{\overbar}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}
\newcommand{\alon}[1]{\footnote{#1 (alon)}}
\newcommand{\todo}[1]{{\color{red}\bf TODO: #1}}
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}




% disjoint union
\makeatletter
\def\moverlay{\mathpalette\mov@rlay}
\def\mov@rlay#1#2{\leavevmode\vtop{%
   \baselineskip\z@skip \lineskiplimit-\maxdimen
   \ialign{\hfil$\m@th#1##$\hfil\cr#2\crcr}}}
\newcommand{\charfusion}[3][\mathord]{
    #1{\ifx#1\mathop\vphantom{#2}\fi
        \mathpalette\mov@rlay{#2\cr#3}
      }
    \ifx#1\mathop\expandafter\displaylimits\fi}
\makeatother
\newcommand{\cupdot}{\charfusion[\mathbin]{\cup}{\cdot}}
\newcommand{\bigcupdot}{\charfusion[\mathop]{\bigcup}{\cdot}}

% machine learning
\newcommand{\LZO}{\ell^{0-1}}
\newcommand{\LH}{\ell^{\text{hinge}}} 
\newcommand{\LD}{L_{\cD}}
\newcommand{\LDZO}{L_{\cD}^{0-1}} 
\newcommand{\LDH}{L_{\cD}^{\text{hinge}}} 
\newcommand{\VC}{\mathrm{VCdim}}
\newcommand{\regret}{\textrm{Regret}}

% Real Analysis
\newcommand{\ballr}[3]{B_{#1} ^{#2} (#3)}   % 1-dimension, 2-norm, 3-radius
\newcommand{\ball}[2]{B_{#1} ^{#2}}  % same with radius 1
\newcommand{\inter}{\mathrm{int}}
\newcommand{\cl}{\mathrm{cl}}
\newcommand{\limn}{\lim_{n \rightarrow \infty}} 
\newcommand{\IFF}{\Leftrightarrow}
\newcommand{\indct}[1]{\boldsymbol{1}\!_{\left[ #1 \right]}}


% Convex Analysis
\newcommand{\conv}{\textrm{conv}}

% Linear Algebra
\newcommand{\sym}[1]{\mathbb{S}^{#1}}
\newcommand{\symps}[1]{\mathbb{S}^{#1}_{+}}
\newcommand{\symp}[1]{\mathbb{S}^{#1}_{++}}
\newcommand{\trace}{\mathrm{trace}}
\newcommand{\vect}{\mathrm{vec}}
\newcommand{\trans}{\dagger}
\newcommand{\inner}[1]{\langle #1 \rangle}
\newcommand{\finner}[1]{\langle #1 \rangle}
\newcommand{\fnorm}[1]{\| #1\|_F}
\newcommand{\snorm}[1]{\| #1\|_{\mathrm{sp}}}
\newcommand{\tnorm}[1]{\| #1\|_{\mathrm{tr}}}
\newcommand{\twonorm}[1]{\| #1\|_2}
\newcommand{\onenorm}[1]{\| #1\|_1}
\newcommand{\infnorm}[1]{\| #1\|_\infty}
\newcommand{\dnorm}[1]{\| #1\|_\star}
\newcommand{\nnz}{\mathrm{nnz}}

%boldsymbol
\newcommand{\vtheta}{\boldsymbol{\theta}}
\newcommand{\tL}{\tilde{L}}
\newcommand{\hL}{\hat{L}}





%DeclareMath
\DeclareMathOperator*{\argmin}{argmin} % Declares argmin and ensures super and subscripts are located nicely above/below such as in \min
\DeclareMathOperator*{\argmax}{argmax} % Declares argmin and ensures super and subscripts are located nicely above/below such as in \min
%\DeclareMathOperator*{\prob}{\mathbb{P}} 


% ref
\renewcommand{\eqref}[1]{Equation~(\ref{#1})}
\newcommand{\exref}[1]{Example~(\ref{#1})}
\newcommand{\exeref}[1]{Exercise~(\ref{#1})}
\newcommand{\figref}[1]{Figure~\ref{#1}}
\newcommand{\secref}[1]{Section~\ref{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}
\newcommand{\appref}[1]{Appendix~\ref{#1}}
\newcommand{\thmref}[1]{Theorem~\ref{#1}}
\newcommand{\lemref}[1]{Lemma~\ref{#1}}
\newcommand{\defref}[1]{Definition~\ref{#1}}
\newcommand{\corref}[1]{Corollary~\ref{#1}}
\newcommand{\clref}[1]{Claim~\ref{#1}}
\newcommand{\algref}[1]{Algorithm~\ref{#1}}
\newcommand{\chapref}[1]{Chapter~\ref{#1}}
\newcommand{\remref}[1]{Remark~\ref{#1}}
%\newcommand{\comment}[1]{\textcolor{red}{\textbf{#1}}}




